Why Do Local Methods Solve Nonconvex Problems?

Non-convex optimization is ubiquitous in modern machine learning. Researchers devise non-convex objective functions and optimize them using off-the-shelf optimizers such as stochastic gradient descent and its variants, which leverage the local geometry and update iteratively. Even though solving non-convex functions is NP-hard in the worst case, the optimization quality in practice is often not an issue -- optimizers are largely believed to find approximate global minima. Researchers hypothesize a unified explanation for this intriguing phenomenon: most of the local minima of the practically-used objectives are approximately global minima. We rigorously formalize it for concrete instances of machine learning problems.

==> macro/authornote.tex <==

\def\shownotes{0}  \ifnum\shownotes=1
\newcommand{\authnote}[2]{$\ll$\textsf{\footnotesize #1 notes: #2}$\gg$}
\else
\newcommand{\authnote}[2]{}
\fi

\newcommand{\tnote}[1]{{\color{blue}\authnote{Tengyu}{#1}}}
\newcommand{\FIXME}[1]{{\color{Red}\authnote{Tengyu}{#1}}}
\newcommand{\TODO}[1]{{{\color{red}\authnote{TODO}{#1}}}}
\newcommand{\TMnote}[1]{{\color{blue}\authnote{Tengyu}{#1}}}
\newcommand{\Rnote}[1]{{\color{blue}\authnote{Tengyu}{#1}}}


==> macro/packages.tex <==



==> tools.tex <==
\\\\\\\\

